A Theoretical Survey on Foundation Models

Understanding the inner mechanisms of black-box foundation models (FMs) is essential yet challenging in artificial intelligence and its applications. Over the last decade, the long-running focus has been on their explainability, leading to the development of post-hoc explainable methods to rationalize the specific decisions already made by black-box FMs. However, these explainable methods have certain limitations in terms of faithfulness and resource requirement. Consequently, a new class of interpretable methods should be considered to unveil the underlying mechanisms of FMs in an accurate, comprehensive, heuristic, and resource-light way. This survey aims to review those interpretable methods that comply with the aforementioned principles and have been successfully applied to FMs. These methods are deeply rooted in machine learning theory, covering the analysis of generalization performance, expressive capability, and dynamic behavior. They provide a thorough interpretation of the entire workflow of FMs, ranging from the inference capability and training dynamics to their ethical implications. Ultimately, drawing upon these interpretations, this review identifies the next frontier research directions for FMs.

==> tax.tex <==
\begin{figure}[htbp]
\centering
\scalebox{0.75}{
\begin{forest}
for tree={
    grow=east, % 分支朝东（向右）生长，形成横向的分支结构
    draw, % 绘制每个节点的边框
    rounded corners, % 每个节点的边框设置为圆角
      node options={align=center, minimum width=2cm}, % 节点文本居中对齐，设置相同的最小宽度 % 节点文本居中对齐
    text centered, % 文本在节点内居中显示
    edge={->, thick}, % 每条边使用粗箭头
    edge path={
        \noexpand\path [draw, \forestoption{edge}] (!u.east) -| +(+5pt,0) |- (.child anchor)
        \forestoption{edge label};
    },
    s sep+=1pt % 增加每个节点之间的水平间距
 %   baseline=1pt
}
[
    Interpretation for FMs, text width=2cm, minimum width=0.5cm, minimum height=0.5cm 
    [Ethic Implications - Section \ref{sec5}
        [Hallucination
            [Detection of hallucination \cite{dhuliawala2023chain,chen2024inside,huang2024opera,cohen2023lm,shi2022natural,wang2022self}, fill=orange!5]
            [Cause of hallucination \cite{xu2024hallucination}, fill=orange!5]
        ]
        [Unfair prediction
            [Generalization analysis \cite{yoon2020joint,pham2023fairness,singh2019fairness,chen2022fairness,schumann2019transfer}, fill=orange!5]
            [Evaluation metric \cite{calders2009building,hardt2016equality}, fill=orange!5]
        ]
        [Privacy leakage
            [Differential privacy and generalization \cite{bagdasaryan2019differential,he2020tighter,ma2022dimension, nissim2015generalization,oneto2017differential,yu2021differentially,ding2024delving,zhang2024dpzero,li2022does,malladi2023fine}, fill=orange!5]
            [Memorization and generalization \cite{feldman2020does}, fill=orange!5]
        ]
    ]
    [Training Process - Section \ref{sec4}
         [Reinforcement Learning from Human Feedback, text width=4cm
          [Online RLHF \cite{xu2020preference, chen2022human,wang2023rlhf, novoseller2020dueling, saha2023dueling,zhan2023query}, fill=orange!5
          ]
          [Offline RLHF \cite{zhu2023principled,zhan2023provable,li2023reinforcement}, fill=orange!5
          ]
          [Dueling Bandits \cite{yue2012k,saha2021optimal}, fill=orange!5]
          ]
         [Parameter Evolution 
          [Training Dynamics \cite{tian2023joma, tian2024scan,abbe2024transformers, li2023transformershow, tarzanagh2023transformers,ataee2023max,jelassi2022vision}, fill=orange!5]
         ]
         [Emergent Capability
             [Quantify Emergence \cite{chen2024quantifying,srivastava2022beyond}, fill=orange!5]
             [Triggers of Emergence \cite{arora2023theory, schaeffer2024emergent},  fill=orange!5]
         ]
    ]
    [Inference Capability - Section \ref{sec3}
       [Distribution Shifts
          [Covariate Shifts ${\mathcal{D}}_{x}^{\text{train }} \neq {\mathcal{D}}_{x}^{\text{test }}$ \cite{zhang2024trained, linonlinear}, fill=orange!5 % 子节点 "Covariate Shifts"，使用浅蓝色填充
          ]
          [Query Shifts ${\mathcal{D}}_{\text{query }}^{\text{test }} \neq {\mathcal{D}}_{x}^{\text{test }}$ \cite{zhang2024trained}, fill=orange!5 % 子节点 "Query Shifts"，使用浅红色填充
          ]
          [Task Shifts ${\mathcal{D}}_{\mathcal{H}}^{\text{train }} \neq {\mathcal{D}}_{\mathcal{H}}^{\text{test }}$ \cite{li2023transformers,zhang2024trained,wies2024learnability,huangcontext, ahn2024transformers}, fill=orange!5 % 子节点 "Task Shifts"，使用浅橙色填充
          % 子节点
          ]
       ]
       [Chain-of-Thought
          [Expressivity Analysis of CoT \cite{feng2024towards,lichain, li2024dissecting,merrill2023expressive}, fill=orange!5]
          [Generalization Analysis for CoT \cite{li2024nonlinear}, fill=orange!5]
       ]
       [In-Context Learning, text width=2cm
            [Expressivity Analysis, text width=2cm
              [ Expressivity of ICL
              \cite{akyurek2022learning, von2023transformers, dai2022can, bai2024transformers,mahankali2023one}, fill=orange!5
              ]
             ]
            [Generalization Analysis, text width=2cm, minimum width=0.1cm, minimum height=0.5cm 
                [Algorithmic Stability \cite{li2023transformers,deoraoptimization}, fill=orange!5]
                [PAC-Bayes arguments \cite{zhang2023and}, fill=orange!5] 
                [Covering numbers \cite{bai2024transformers,lintransformers}, fill=orange!5]
                [Gradient Flow Based  \cite{wu2023many,liu2024towards,nichani2024transformers}, fill=orange!5] 
            ]
       ]
    ]
]
\end{forest}
}
\caption{The overall structure of the survey} % 图表标题
\label{fig:overviewdiagram} % 图表标签，用于引用
\end{figure}

==> taxonomy.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \vspace{-1.0cm}
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=4em,font=\normalsize,}{},
            where level=2{text width=7.5em,font=\normalsize,}{},
            where level=3{text width=6.0em,font=\normalsize,}{},
            where level=4{text width=6.0em,font=\normalsize,}{},
            [
                In-context Learning, ver
                [
                    Training, ver
                    [
                        Pre-training (\S \ref{sec:pretraining})
                        [
                         PICL~\cite{picl}{, }MEND~\cite{Li2023mend}{, }ICLM~\cite{Shi2023iclm}, leaf, text width=45.0em
                        ]
                    ]
                    [
                        Warmup (\S \ref{sec:warmup})
                        [
                            MetaICL~\cite{metaicl}{, }OPT-IML~\cite{optiml}{, }Super-NaturalInstructions~\cite{natural}{, }\\FLAN~\cite{flan}{, }Scaling Instruction~\cite{chung}{, }Self-supervised ICL~\cite{selfsupericl}{, }\\Symbol Tuning~\cite{symboltuning}{, }RICL~\cite{Chu2023Finetune}
                                {, }ICL Markup~\cite{Brunet2023Markup}, leaf, text width=45.0em
                        ]
                    ]
                ]    
                [
                    Inference, ver
                    [
                        Demonstration\\ (\S \ref{sec:demonstration_org})
                        [       
                           Selection \\ (\S \ref{sec:select})
                                [
                                    Unsupervised
                                    [
                                       KATE~\cite{liu2022close}{, }SG-ICL~\cite{kim2022self}{, }Self-Adaptive\\\cite{Wu2022SelfadaptiveIL}{, }PPL~\cite{gonen2022demystifying}{, }MI~\cite{sorensen2022information}{, }\\Informative Score~\cite{li2023supporting}{, }IDS~\cite{qin2023incontext}{,}\\Votek~\cite{su2022selective}
                                        , leaf, text width=29.7em
                                    ]
                                ] 
                                [
                                    Supervised
                                    [
                                      EPR~\cite{rubin2022learning}{, }Q-Learning~\cite{zhang2022active}{, }\\AdaICL~\cite{mavromatis2023examples}{, }Topic~\cite{topic}{, }\\UDR~\cite{udr}
                                        , leaf, text width=29.7em
                                    ]
                                ]
                        ]
                        [
                            Reformatting \\ (\S \ref{sec:reformatting})
                            [   
                            SG-ICL~\citep{kim2022self}{, }Structrured Prompting~\cite{hao2022structured}{, }\\AutoICL~\citep{yang2023autoicl}{, }WICL~\citep{yang2023demonstration}{, }ICV~\citep{liu2024incontext}, leaf, text width=37.3em
                            ]
                        ]
                        [
                            Ordering \\ (\S \ref{sec:order})
                            [ GlobalE\&LocalE~\cite{lu2022order}{,} ICCL~\cite{liu2024lets}
                            , leaf, text width=37.3em
                            ]
                        ]
                    ]
                    [
                        Instruction (\S \ref{sec:instruction})
                        [
                            Instruction Induction~\cite{induct}{, }Self-Instruct~\cite{wang2022self}{, }APE~\cite{zhou2022large}{, }\\Grimoire~\cite{chen2024grimoire}
                                , leaf, text width=45.0em
                        ]
                    ]
                    [
                        Scoring \\ Function (\S \ref{sec:scoring})
                        [
                            Calibrate~\cite{calibrate}{, }Channel Models~\cite{min2022noisy}{, }$k$NN-Prompting~\citep{knnPrompting}, leaf, text width=45.0em
                        ]
                    ]
                ]
                [
                Analysis, ver
                    [
                        Influencing \\Factors  (\S \ref{sec:inf_factors})
                        [ Pre-training \\Stage (\S \ref{sec:inf_factors_pre})
                            [Pre-Training\\ Data
                                [Distribution~\cite{distribution,wies2024learnability}{, }Domain\\\cite{shin2022corpora, Han2023UnderstandingIL}{, }Diversity~\cite{Yadlowsky2023PretrainingDM}, leaf, text width=29.6em
                                ]
                            ]
                            [Model and\\Training
                                [Architecture
                            ~\cite{Ding2023CausalLMIN}{, }Pre-training steps~\cite{wei2022emergent}{, }\\Parameters~\cite{gpt3,wei2022emergent},
                          leaf, text width=29.6em
                                ]
                            ]
                        ]
                        [ Inference\\ Stage (\S \ref{sec:inf_factors_infe})
                            [ Input Labels
                                [
                                Mapping~\cite{ground_truth,Pan2023WhatIL,Tang2023LargeLM}{, }\\Settings~\cite{min2022rethinking},
                          leaf, text width=29.6em
                                ]
                            ]
                            [Demonstration\\ Examples
                                [Diversity and Simplicity~\cite{compositional_generalization}{, }Query Similarity\\\cite{liu2022close, compositional_generalization}{, }Feature bias~\cite{inductive_bias}{, }\\Order~\cite{lu2022order, Zhang2022ActiveES,Liu2023LostIT},
                          leaf, text width=29.6em
                                ]
                            ]
                        ]
                    ]
                    [
                        Learning \\Mechanism (\S \ref{sec:mech}) 
                        [ Functional\\ Modules\\(\S \ref{sec:mech_fun})       
                            [
                            Induction Heads~\cite{olsson2022induction, Bietti2023BirthOA}
                        {, }\\Computational Layers~\cite{label_anchor}{, }Attention Modules~\cite{icl_weight_shifting},
                        % , Gao2023InContextLF, zhang2023and
                          leaf, text width=37.3em
                            ]
                        ]
                        [ 
                            Theoretical\\ Interpretation\\(\S\ref{sec:mech_theo})
                            [
                                Bayesian Framework                                      ~\cite{bayesian, topic, jiang2023latent}{, }\\Gradient Descent~\cite{dai2022iclft, Irie2022TheDF, mahankali2023one}{, }\\Others~\cite{garg2022linear, akyurek2022algorithm, trm_as_alg, tr_and_tl}, leaf, text width=37.3em    
                            ]
                        ]
                    ]
                ]  
            ]
        \end{forest}
    }
    \caption{Taxonomy of in-context learning.}
    \label{taxo_of_icl}
\end{figure*}

